Convolutional Self-Attention-Based Multi-User MIMO Demapper

In orthogonal frequency division multiplexing (OFDM)-based wireless communication systems, the bit error rate (BER) performance is heavily dependent on the accuracy of channel estimation. It is important for a good channel estimator to be capable of handling the changes in the wireless channel conditions that occur due to the mobility of the users. In recent years, the focus has been on developing complex neural network (NN)- based channel estimators that enable an error performance close to that of a genie-aided channel estimator. This work considers the other alternative which is to have a simple channel estimator but a more complex NN-based demapper for the generation of soft information for each transmitted bit. In particular, the problem of reversing the adverse effects of an imperfect channel estimator is addressed, and a convolutional self-attention-based neural demapper that significantly outperforms the baseline is proposed.

==> figs/ber_cvt.tex <==
% This file was created with tikzplotlib v0.9.12.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
log basis y={10},
tick align=outside,
tick pos=left,
title={Speed: 3.60 km/h},
x grid style={white!69.0196078431373!black},
xlabel={SNR [dB]},
xmajorgrids,
xmin=10, xmax=31,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={BER},
ymajorgrids,
ymin=6e-05, ymax=0.5,
ymode=log,
ytick style={color=black},
ytick={1e-06,1e-05,0.0001,0.001,0.01,0.1,1,10},
yticklabels={
  \(\displaystyle {10^{-6}}\),
  \(\displaystyle {10^{-5}}\),
  \(\displaystyle {10^{-4}}\),
  \(\displaystyle {10^{-3}}\),
  \(\displaystyle {10^{-2}}\),
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\),
  \(\displaystyle {10^{1}}\)
}
]
\addplot [very thin, color0, mark=asterisk, mark size=2.5, mark options={solid}]
table {%
10 0.0030989577062428
13.5 0.000832519261166453
17 0.000222167960600927
20.5 4.39453033322934e-05
24 0
27.5 0
31 0
};
\addlegendentry{Perfect CSI - Gaussian demapper}
\addplot [very thin, color1, mark=x, mark size=2.5, mark options={solid}]
table {%
10 0.0719719752669334
13.5 0.0432301536202431
17 0.0233072638511658
20.5 0.00991629995405674
24 0.00357251078821719
27.5 0.000934163574129343
31 0.000359456287696958
};
\addlegendentry{Baseline}
\addplot [very thin, color2, mark=diamond*, mark size=2.5, mark options={solid}]
table {%
10 0.00940040219575167
13.5 0.00327803078107536
17 0.00115610437933356
20.5 0.000356738368282095
24 8.85741537786089e-05
27.5 2.32910369959427e-05
31 6.44531473881216e-06
};
\addlegendentry{CvT Demapper}
\end{axis}

\end{tikzpicture}

